Single Image Depth Prediction with Wavelet Decomposition

We present a novel method for predicting accurate depths from monocular images with high efficiency. This optimal efficiency is achieved by exploiting wavelet decomposition, which is integrated in a fully differentiable encoder-decoder architecture. We demonstrate that we can reconstruct high-fidelity depth maps by predicting sparse wavelet coefficients. In contrast with previous works, we show that wavelet coefficients can be learned without direct supervision on coefficients. Instead we supervise only the final depth image that is reconstructed through the inverse wavelet transform. We additionally show that wavelet coefficients can be learned in fully self-supervised scenarios, without access to ground-truth depth. Finally, we apply our method to different state-of-the-art monocular depth estimation models, in each case giving similar or better results compared to the original model, while requiring less than half the multiply-adds in the decoder network. Code at https://github.com/nianticlabs/wavelet-monodepth

==> figure_results.tex <==
\begin{figure*}[ht]
\centering
\setlength\lineskip{0pt}
\setlength\tabcolsep{0pt} 
\begin{tabular}{ccc}
    \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png} & \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png} & 
    \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png}\\
    \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png} & \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png} & 
    \includegraphics[width=.33\linewidth, valign=b]{images/coefficients_tmp.png}\\
\end{tabular}
    \caption{A placeholder for the big figure with qualitative results on the KITTI dataset}
    \label{fig:qualitative_results}
\end{figure*}

==> images/wavelet_vis/figure_wavelets.tex <==
\begin{figure*}[!ht]
\centering
\setlength\lineskip{1pt}
\setlength\tabcolsep{0pt} 
\begin{center}
\begin{tabular}{>{\centering\arraybackslash}m{0.082\textwidth} 
>{\centering\arraybackslash}m{0.153\textwidth}
>{\centering\arraybackslash}m{0.153\textwidth}
>{\centering\arraybackslash}m{0.153\textwidth}
>{\centering\arraybackslash}m{0.153\textwidth}
>{\centering\arraybackslash}m{0.153\textwidth}
>{\centering\arraybackslash}m{0.153\textwidth}
}
% ~ & ~ & KITTI~\cite{Geiger2012CVPR} ~ &~ & ~ & NYUv2~\cite{Nyuv2} ~ &\\
% RGB input & 

RGB & 
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_rgb.png}
\end{subfigure} \\

LL3 & 
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_LL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_LL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_LL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_LL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_LL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_LL.png}
\end{subfigure} \\

LH &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_LH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_LH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_LH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_LH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_LH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_LH.png}
\end{subfigure} \\

HL & 
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_HL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_HL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_HL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_HL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_HL.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_HL.png}
\end{subfigure} \\

HH & 
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_HH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_HH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_HH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_HH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_HH.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_HH.png}
\end{subfigure} \\

Final &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/2_pred.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/132_pred.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/653_pred.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/235_pred.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/244_pred.png}
\end{subfigure} &
\begin{subfigure}[b]{0.153\textwidth}
     \centering
     \includegraphics[width=\textwidth]{images/qualitative_nyu/wavelets_decompositions/555_pred.png}
\end{subfigure} \\
\end{tabular}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Qualitative results of predicted wavelets coefficients of depth maps on the NYU dataset}. Our predicted wavelets have two desirable properties: they are sparse, allowing for efficient computation, and they are accurately located around depth edges without needing to supervise them.}
    \label{fig:qualitative_wavelets}
\end{figure*}

==> string.tex <==
@STRING{AI       = "Artificial Intelligence"}
@STRING{AAAI     = "American Association for Artificial Intelligence Conference"}
@STRING{ACC      = "American Control Conference"}
@STRING{ACCV     = "Asian Conference on Computer Vision"}
@STRING{ACM      = "Association for Computing Machinery"}
@STRING{AISTATS  = "International Conference on Artificial Intelligence and Statistics"}
@STRING{ARXIV    = "arXiv Preprint"}
@STRING{AVSS     = "International Conference on Advanced Video and Signal Based Surveillance"}
@STRING{BIOINF   = "Bioinformatics"}
@STRING{BMVC     = "British Machine Vision Conference"}
@STRING{CA       = "Computer Animation"}
@STRING{CACM     = "Communications of the ACM"}
@STRING{CAD      = "Computer Aided Design Journal"}
@STRING{CAIP     = "Computer Analysis of Images and Patterns"}
@STRING{CG       = "Computers \& Graphics"}
@STRING{CGA      = "Computer Graphics and Applications"}
@STRING{CGF      = "Computer Graphics Forum"}
@STRING{CGI      = "Computer Graphics International"}
@string{CGIP     = "Computer Graphics and Image Processing"}
@string{CHI      = "ACM Conference on Human Factors in Computing Systems"}
@string{CIARP    = "Iberoamerican Congress on Pattern Recognition"}
@string{CIKM     = "Conference on Information and Knowledge Management"}
@string{COLT     = "Conference on Computational Learning Theory"}
@string{CORR     = "Computing Research Repository"}
@string{CPAM     = "Communications on Pure and Applied Mathematics"}
@string{CIVR     = "Conference on Image and Video Retrieval"}
@string{CSUR     = "ACM Computing Surveys"}
@string{CVBIA    = "Workshop on Computer Vision for Biomedical Image Applications"}
@string{CVGIP    = "Computer Vision, Graphics, and Image Processing"}
@string{CVIU     = "Computer Vision and Image Understanding"}
@STRING{CVPR     = "Conference on Computer Vision and Pattern Recognition"}
@STRING{CVPRW    = "Conference on Computer Vision and Pattern Recognition Workshops"}
@STRING{CVWW     = "Computer Vision Winter Workshop"}
@STRING{DAGM     = "DAGM Symposium on Pattern Recognition"}
@STRING{DICTA    = "Digital Image Computing: Techniques and Applications"}
@STRING{ECAI     = "European Conference on Artificial Intelligence"}
@STRING{ECCTD    = "European Conference on Circuit Theory and Design"}
@STRING{ECCV     = "European Conference on Computer Vision"}
@STRING{ECCVW    = "European Conference on Computer Vision Workshops"}
@STRING{ECML     = "European Conference on Machine Learning"}
@STRING{EG       = "Eurographics"}
@STRING{FGR      = "Automated Face and Gesture Recognition"}
@STRING{FTCGV    = "Foundations and Trends in Computer Graphics and Vision"}
@STRING{FTML     = "Foundations and Trends in Machine Learning"}
@STRING{IA       = "Image Analysis"}
@STRING{IAPRS    = "International Archives of Photogrammetry and Remote Sensing"}
@STRING{ICANN    = "International Conference on Artificial Neural Networks"},
@STRING{ICASSP   = "International Conference on Acoustics, Speech, and Signal Processing"}
@STRING{ICBI     = "International Conference on Biomedical Imaging"}
@STRING{ICCV     = "International Conference on Computer Vision"}
@STRING{ICCVW    = "International Conference on Computer Vision Workshops"}
@STRING{ICCVTA   = "International Conference on Computer Vision Theory and Applications"}
@STRING{ICIAP    = "International Conference on Image Analysis and Processing "}
@STRING{ICIP     = "International Conference on Image Processing"}
@STRING{ICIRS    = "International Conference on Intelligent Robots and Systems"}
@STRING{ICLR     = "International Conference for Learning Representations"}
@STRING{ICML     = "International Conference on Machine Learning"}
@STRING{ICME     = "International Conference on Multimedia and Expo"}
@STRING{ICONIP   = "International Conference on Neural Information Processing"}
@STRING{ICPR     = "International Conference on Pattern Recognition"}
@STRING{ICRA     = "International Conference on Robotics and Automation"}
@STRING{ICVGIP   = "Indian Conference on Computer Vision, Graphics and Image Processing"}
@STRING{IJBI     = "International Journal of Biomedical Imaging"}
@STRING{IJCAI    = "International Joint Conference on Artificial Intelligence"}
@STRING{IJCNN    = "International Joint Conference on Neural Networks"}
@STRING{IJCV     = "International Journal of Computer Vision"}
@STRING{IJBI     = "International Journal of Biomedical Imaging"}
@STRING{IJMI     = "International Journal of Medical Informatics"}
@STRING{IJPRAI   = "International Journal of Pattern Recognition and Artificial Intelligence"}
@STRING{IJRR     = "International Journal of Robotics Research"}
@STRING{IJPRS    = "International Journal of Photogrammetry and Remote Sensing"}
@STRING{IPMI     = "Information Processing in Medical Imaging"}
@STRING{IPSN     = "Information Processing in Sensor Networks"}
@STRING{IROS     = "International Conference on Intelligent Robots and Systems"}
@STRING{ISBI     = "International Symposium on Biomedical Imaging"}
@STRING{ISMAR    = "International Symposium on Mixed and Augmented Reality"}
@STRING{ISCIS    = "International Symposium on Computer and Information Sciences"}
@STRING{ISPRS    = "International Society for Photogrammetry and Remote Sensing"}
@STRING{IU       = "DARPA Image Understanding Workshop"}
@STRING{IVC      = "Image and Vision Computing"}
@STRING{ISIT     = "International Symposium on Information Theory"}
@STRING{JAIR     = "Journal of Artificial Intelligence Research"}
@STRING{JCB      = "Journal of Cell Biology"}
@STRING{JB       = "Journal of Biomechanics"}
@STRING{JEA      = "Journal on Experimental Algorithmics"}
@STRING{JIVC     = "Journal of Image and Vision Computing"}
@STRING{JMIV     = "Journal of Mathematical Imaging and Vision"}
@STRING{JMLR     = "Journal of Machine Learning Research"}
@STRING{JNM      = "Journal of Neuroscience Methods"}
@STRING{JRA      = "Journal of Robotics and Automation"}
@STRING{JRSS     = "Journal of the Royal Statistical Society"}
@STRING{JSB      = "Journal of Structural Biology"}
@STRING{JVCA     = "Journal of Visualization and Computer Animation"}
@STRING{JVCIR    = "Journal of Visual Communication and Image Representation"}
@STRING{KDD      = "Conference on Knowledge Discovery and Data Mining"}
@STRING{MEDIA    = "Medical Image Analysis"}
@STRING{MICCAI   = "Conference on Medical Image Computing and Computer Assisted Intervention"}
@STRING{MIA      = "Medical Image Analysis"}
@STRING{MIG      = "Motion in Games"}
@STRING{MIV      = "Journal of Mathematical Imaging and Vision"}
@STRING{ML       = "Machine Learning"}
@STRING{MLMI     = "Machine Learning in Medical Imaging"}
@STRING{MMBIA    = "Workshop on Mathematical Methods in Biomedical Image Analysis"}
@STRING{MRI      = "Magnetic Resonance in Medicine"}
@STRING{MVA      = "Machine Vision and Applications"}
@STRING{NATURE   = "Nature"}
@STRING{NATMET   = "Nature Methods"}
@STRING{NEURINF  = "Neuroinformatics"}
@STRING{NEM      = "New European Media"}
@STRING{NEURIMG  = "NeuroImage"}
@STRING{NEM      = "New European Media"}
@STRING{NIPS     = "Advances in Neural Information Processing Systems"}
@STRING{NORDIA   = "CVPR Workshop on Non-Rigid Shape Analysis and Deformable Image Alignment"}
@STRING{PAMI     = "IEEE Transactions on Pattern Analysis and Machine Intelligence"}
@STRING{PERS     = "Journal of Photogrammetry Engineering and Remote Sensing"}
@STRING{PETS     = "IEEE International Workshop on Performance Evaluation of Tracking and Surveillance"}
@STRING{PIEEE    = "Proceedings of the IEEE"}
@STRING{PLOS1    = "PloS one"}
@STRING{PNAS     = "Proceedings of the National Academy of Sciences USA"}
@STRING{PR       = "Pattern Recognition"}
@STRING{PRL      = "Pattern Recognition Letters"}
@STRING{PRSB     = "Proceedings Royal Society London, Biology" }
@STRING{RFIA     = "Reconnaissance des Formes et Intelligence Artificielle"}
@STRING{RSS      = "Robotics: Science and Systems Conference"}
@STRING{SCA      = "ACM Symposium on Computer Animation"}
@STRING{SCIA     = "Scandinavian Conference on Image Analysis"}
@STRING{SCIENCE  = "Science"}
@STRING{SCIPY    = "Python for Scientific Computing Conference"}
@STRING{SIGGRAPH = "ACM SIGGRAPH"}
@STRING{SIGIR    = "ACM SIGIR proceedings on Research and Development in Information Retrieval"}
@STRING{SMC      = "IEEE Transactions on Systems, Man, and Cybernetics"}
@STRING{SPIE     = "SPIE"}
@STRING{TVCG     = "IEEE Transactions on Visualization and Computer Graphics"}
@STRING{TBME     = "IEEE Transactions on Biomedical Engineering"}
@STRING{TCSVT    = "IEEE Transactions on Circuits and Systems for Video Technology"}
@STRING{TDPVT    = "3D Data Processing, Visualization and Transmission"}
@STRING{TIP      = "IEEE Transactions on Image Processing"}
@STRING{TIST     = "ACM Transactions on Intelligent Systems and Technology"}
@STRING{TIT      = "IEEE Transactions on Information Theory"}
@STRING{TITB     = "Transactions on Information Technology in Biomedicine"}
@STRING{TMI      = "IEEE Transactions on Medical Imaging"}
@STRING{TNN      = "IEEE Transactions on Neural Networks"}
@STRING{TVCG     = "IEEE Transactions on Visualization and Computer Graphics"}
@STRING{TVLSI    = "IEEE Transactions on VLSI Systems"}
@STRING{TMS      = "ACM Transactions on Mathematical Software"}
@STRING{TOG      = "ACM Transactions on Graphics"}
@STRING{TOMS     = "ACM Transactions on Mathematical Software"}
@STRING{TRA      = "IEEE Transactions on Robotics and Automation"}
@STRING{TSP      = "IEEE Transactions on Signal Processing"}
@STRING{UAI      = "Uncertainty in Artificial Intelligence"}
@STRING{UIST     = "User Insterface Software and Technology Symposium"}
@STRING{VISU     = "IEEE Conference on Visualization "}
@STRING{VRST     = "ACM Symposium on Virtual Reality Software and Technology"}
@STRING{VMW      = "International Workshop on Vision, Modeling and Visualization"}
@STRING{VCIP     = "SPIE International Conference on Visual Communications and Image Processing"}
@STRING{WACV     = "IEEE Winter Conference on Applications of Computer Vision"}
 

==> sup_mat_figure_qualitative.tex <==
\begin{figure*}[!ht]
\centering
\setlength\lineskip{1pt}
\setlength\tabcolsep{0pt} 
\begin{center}
\begin{tabular}{>{\centering\arraybackslash}m{6em} 
>{\centering\arraybackslash}m{0.17\textwidth}
>{\centering\arraybackslash}m{0.17\textwidth}
>{\centering\arraybackslash}m{0.17\textwidth}@{\hskip 0.08in}
>{\centering\arraybackslash}m{0.11\textwidth}
>{\centering\arraybackslash}m{0.11\textwidth}
>{\centering\arraybackslash}m{0.11\textwidth}
}
~ & ~ & KITTI~\cite{Geiger2012CVPR} ~ &~ & ~ & NYUv2~\cite{Nyuv2} ~ &\\
RGB input & 
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_rgb.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_rgb.png}
\end{subfigure}\\

\multirow{2}{*}{LL3 only} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_LL3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_LL3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_LL3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_LL3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_LL3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_LL3.png}
\end{subfigure}\\
~ & 
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_LL3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_LL3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_LL3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_LL3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_LL3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_LL3_error.png}
\end{subfigure}\\

\multirow{2}{*}{LL3 + H3} & 
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_LL3_H3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_LL3_H3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_LL3_H3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_LL3_H3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_LL3_H3.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_LL3_H3.png}
\end{subfigure}\\
~ &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_LL3_H3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_LL3_H3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_LL3_H3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_LL3_H3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_LL3_H3_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_LL3_H3_error.png}
\end{subfigure}\\
% LL3 + H3 + H2 &
% \begin{subfigure}[b]{0.8\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, valign=b]{images/ablate_LL3_H3H2.png}
% \end{subfigure}\\
% LL3 + all HF ($\eta$=0.1) &
% \begin{subfigure}[b]{0.8\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, valign=b]{images/ablate_sparsity_1e-1.png}
% \end{subfigure} \\


\multirow{2}{*}{\shortstack[lb]{LL3 + all HF \\ $\psi < 20\%$}} & 
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_sparsity_0.10.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_sparsity_0.10.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_sparsity_0.10.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_sparsity_0.2.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_sparsity_0.2.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_sparsity_0.2.png}
\end{subfigure}\\
% (K~\cite{Geiger2012CVPR}: $\eta < 10\%$, N~\cite{Nyuv2}: $\eta < 20\%$)  
~
&
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/0_sparsity_0.10_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/431_sparsity_0.10_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.17\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_kitti/427_sparsity_0.10_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/299_sparsity_0.2_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/348_sparsity_0.2_error.png}
\end{subfigure} &
\begin{subfigure}[b]{0.11\textwidth}
     \centering
     \includegraphics[width=\textwidth, height=1.3cm]{images/qualitative_nyu/333_sparsity_0.2_error.png}
\end{subfigure}\\
\end{tabular}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Additional qualitative results on wavelet representation of depth maps}. When using only a subset of wavelet scales, we run the inverse wavelet transform up to the highest scale with those coefficients, then perform a bilinear upsampling up to the full resolution. For each experiment, the bottom line shows the $\ell_1$ error map between the considered depth maps and the depth map reconstructed with the complete set of predicted wavelet coefficients.}
    \label{fig:sup_mat_sparsity_qual}
\end{figure*}

==> tables/architectures/waveconv_nyu.tex <==
\begin{table}[t]
  \centering
  \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}[t]{|l|l|l|l|l|l|l|}
        \hline
        \multicolumn{7}{|l|}{\textbf{disp4 Layer}} \\
        \hline
        \textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input}   & \textbf{activation}    \\ \hline
        disp4       & 3      & 1     & 1  & 16 & iconv5 & Linear\\
        \hline
        \multicolumn{7}{l}{~} \\
        \hline
        \multicolumn{7}{|l|}{\textbf{Wavelet Decoding Layer - waveJ}} \\
        \hline
        \textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{res} & \textbf{input}   & \textbf{activation}    \\ \hline
        wave\textbf{J}(1+)       & 1      & 1      & \textbf{chns}(iconv[\textbf{J}+1])      & $2^{\boldsymbol{J}+1}$   & iconv[\textbf{J}+1]                     & LeakyReLU(0.1) \\
        wave\textbf{J}(2+)       & 3      & 1      & 3  & $2^{\boldsymbol{J}+1}$   & wave\textbf{J}(1+) & Sigmoid \\ \hline
        wave\textbf{J}(1-)       & 1      & 1      & \textbf{chns}(iconv[\textbf{J}+1])      & $2^{\boldsymbol{J}+1}$   & iconv[\textbf{J}+1]                     & LeakyReLU(0.1) \\
        wave\textbf{J}(2-)       & 3      & 1      & 3  & $2^{\boldsymbol{J}+1}$   & wave\textbf{J}(1-) & Sigmoid \\ \hline
        \multirow{2}{*}{substract} & \multirow{2}{*}{1} & \multirow{2}{*}{1} & \multirow{2}{*}{3} & \multirow{2}{*}{$2^{\boldsymbol{J}+1}$} & wave\textbf{J}(2+), & \multirow{2}{*}{Linear} \\
        ~ & ~ & ~ & ~ & ~ & wave\textbf{J}(2-) & ~\\
        \hline
    \end{tabular}
    }
  \vspace{2pt}
  \caption{\textbf{Architecture of our wavelet decoding layer used for NYU experiments} J denotes the level of the decoder. \textbf{disp4} is used produce the low-resolution estimate \lli{3}, while \textbf{waveJ} is used to decode $\{\text{\lhi{\textbf{J}}}, \text{\hli{\textbf{J}}}, \text{\hhi{\textbf{J}}}\}$.
%   For experiments on the NYUv2 dataset~\cite{Nyuv2} we only used one convolution layer with \textbf{s}=1 and \textbf{k}=3, without output activation.
  } 
  \vspace{40pt}
\label{tab:waveconv_NYU}
\end{table}

==> tables/occlusion_boundary.tex <==
\begin{table*} %[!ht]
    \centering
    \footnotesize
    \begin{tabular}{|l||c|c|}
    \hline
        Wavelets & $\epsilon_{acc} (\downarrow)$ & $\epsilon_{comp} (\downarrow)$ \\ \hline
        LL only &   9.020  &   9.916\\ \hline
        [3] &   4.197 &   9.154\\ \hline
        [3, 2] &   2.513  &   8.378\\ \hline
        [3, 2, 1] &   2.115  &   7.959 \\\hline
    \end{tabular}
    \vspace{-4pt}
    \caption{\textbf{Ablation study on wavelet coefficients for sharp depth edges} We can see that adding wavelets more levels of wavelet coefficients gradually improves the sharpness of depth maps, as they add high frequency details to the low-resolution estimate. Results are computed using our DenseNet161 based model.}
    \label{tab:ablation_study_edges}
    \vspace{-12pt}
\end{table*}
